Uniform Information Segmentation

Size uniformity is one of the main criteria of superpixel methods. But size uniformity rarely conforms to the varying content of an image. The chosen size of the superpixels therefore represents a compromise - how to obtain the fewest superpixels without losing too much important detail. We propose that a more appropriate criterion for creating image segments is information uniformity. We introduce a novel method for segmenting an image based on this criterion. Since information is a natural way of measuring image complexity, our proposed algorithm leads to image segments that are smaller and denser in areas of high complexity and larger in homogeneous regions, thus simplifying the image while preserving its details. Our algorithm is simple and requires just one input parameter - a threshold on the information content. On segmentation comparison benchmarks it proves to be superior to the state-of-the-art. In addition, our method is computationally very efficient, approaching real-time performance, and is easily extensible to three-dimensional image stacks and video volumes.

==> tex/00_teaser.tex <==
%----------------------------------------------------------------
%\newcommand{\gap}{@{\hspace{.5mm}}}
\newcommand{\teasercolwidth}{0.23\linewidth}%set the column width here
%----------------------------------------------------------------

\begin{figure*}[htbp]
\centering
%\begin{tabular}{@{}c@{}c@{}c@{}c@{}c}
\begin{tabular}{c c c c}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\includegraphics[width=\teasercolwidth]{images/teaser/172032.jpg}&
%\includegraphics[width=\teasercolwidth]{images/teaser/66075.jpg}&
%\includegraphics[width=\teasercolwidth]{images/teaser/198004.jpg}&
%\includegraphics[width=\teasercolwidth]{images/teaser/225017.jpg}\\
\includegraphics[width=\teasercolwidth]{images/teaser/172032_scadq.png}&
\includegraphics[width=\teasercolwidth]{images/teaser/66075_scadq.png}&
\includegraphics[width=\teasercolwidth]{images/teaser/198004_scadq.png}&
\includegraphics[width=\teasercolwidth]{images/teaser/225017_scadq.png}\\
%
% \includegraphics[width=\teasercolwidth]{images/teaser/353013_scadq.png}&
% \includegraphics[width=\teasercolwidth]{images/teaser/253036_scadq.png}&
% \includegraphics[width=\teasercolwidth]{images/teaser/156079_scadq.png}&
% \includegraphics[width=\teasercolwidth]{images/teaser/295087_scadq.png}\\

\end{tabular}
\caption{Images segmented with the Adaptels algorithm (a termination threshold of 60 was used for all the images). Notice how the segments adhere to the object boundaries, adapt to the scale, and remain compact and smooth at the boundaries. These properties make it a unique algorithm that has many applications.}
\label{fig:teaser}
%\vspace{-6mm}
\end{figure*}

==> tex/50_fig_viscomp.tex <==
%----------------------------------------------------------------
\newcommand{\viscompcolwd}{0.16\linewidth}%set the coloumn width here
%\newcommand{\gap}{@{\hspace{.5mm}}}
%----------------------------------------------------------------
\begin{figure*}
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_egb.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_tpix.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_slic.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_seeds.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_ers.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_scad.png}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_egb_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_tpix_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_slic_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_seeds_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_ers_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_246016_3_scad_zoomin.png}\\

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_egb.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_tpix.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_slic.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_seeds.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_ers.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_scad.png}\\

% %
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_egb_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_tpix_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_slic_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_seeds_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_ers_zoomin.png}&
% \includegraphics[width=\viscompcolwd]{images/gtblend/500_163014_8_scad_zoomin.png}\\

\includegraphics[width=\viscompcolwd]{images/gtblend/500_208001_0_egb.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_208001_0_tpix.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_208001_0_slic.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_208001_0_seeds.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_208001_0_ers.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_208001_0_scad.png}\\

\includegraphics[width=\viscompcolwd]{images/gtblend/500_187029_1_egb.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_187029_1_tpix.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_187029_1_slic.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_187029_1_seeds.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_187029_1_ers.png}&
\includegraphics[width=\viscompcolwd]{images/gtblend/500_187029_1_scad.png}\\

%\includegraphics[width=\viscompcolwd]{images/gtblend/500_25098_0_egb.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_25098_0_tpix.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_25098_0_slic.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_25098_0_seeds.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_25098_0_ers.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_25098_0_scad.png}\\

%\includegraphics[width=\viscompcolwd]{images/gtblend/500_100080_0_egb.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_100080_0_tpix.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_100080_0_slic.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_100080_0_seeds.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_100080_0_ers.png}&
%\includegraphics[width=\viscompcolwd]{images/gtblend/500_100080_0_scad.png}\\

\small{(a) EGB~\cite{Felzenszwalb_Huttenlocher_IJCV2004}} & \small{(b) TPIX~\cite{Levenshtein_Kutulakos_Fleet_Dickinson_Siddiqi_PAMI2009}} & \small{(c) SLIC~\cite{Achanta_etal_SLIC_PAMI2012}} & \small{(c) SEEDS~\cite{Bergh_etal_SEEDS_IJCV2015}} & \small{(d) ERS~\cite{Liu_etal_ERS_CVPR2011}} & \small{(e) Adaptels}\\
\end{tabular}
\caption{Visual comparison of different segmentation algorithms. Superpixel boundaries are
overlaid in white on groundtruth segments.
Notice how well Adaptels adapt to each region of the image according to its local structure.
Results for adaptels use a threshold~$T=90\,\textrm{bits}$ and the initial
seed is the central pixel of each image.}
\label{fig:viscomp}
%\vspace{-6mm}
\end{figure*}

==> tex/50_plots_5in1.tex <==
\begin{figure*}
\centering
\begin{tabular}{@{}c@{}c@{}c}
\includegraphics[width=0.33\linewidth]{plots/cuse} &
\includegraphics[width=0.33\linewidth]{plots/recall2} &
\includegraphics[width=0.33\linewidth]{plots/precision2} \\
(a) CUSE & (b) Boundary recall & (c) Boundary precision
%\small{(a) Sum of squared errors computed using Eq.~\ref{eq:sse}.} & \small{(b)Explained variation computed using Eq.~\ref{eq:explainedvariation}.}\\
\end{tabular}
\begin{tabular}{c c}
% \includegraphics[width=0.5\linewidth]{plots/cuse}&
% \includegraphics[width=0.5\linewidth]{plots/recall2}\\
% \small{(a) CUSE}&
% \small{(b) Boundary recall}\\
\includegraphics[width=0.5\linewidth]{plots/prcurve2}&
\includegraphics[width=0.5\linewidth]{plots/fmeasure}\\
\small{(d) Precision versus recall}&
\small{(e) F-measure.}\\
\end{tabular}
%\begin{tabular}{@{}c@{}c@{}c}
%\includegraphics[width=0.33\linewidth]{plots/compactness_schick} &
%\includegraphics[width=0.33\linewidth]{plots/sse} &
%\includegraphics[width=0.33\linewidth]{plots/explainedVariation} \\
%(f) Compactness & (g) SSE & (h) Explained Variation
%\end{tabular}
\caption{Comparison of adaptels to state-of-the-art methods.
(a)~The under-segmentation error of Adaptels is lower than all algorithms. (b)~Adaptels has a lower boundary recall than the state-of-the-art (as explained in main text),
but (c)~a higher precision, and therefore (d)~a better precision-recall curve and (e)~F-measure, the reference measures for any retrieval task.
}
\label{fig:plots}
%\vspace{-15mm}
\end{figure*}
